Information Theory Strikes Back: New Development in the Theory of Cardinality Estimation

Estimating the cardinality of the output of a query is a fundamental problem in database query processing. In this article, we overview a recently published contribution that casts the cardinality estimation problem as linear optimization and computes guaranteed upper bounds on the cardinality of the output for any full conjunctive query. The objective of the linear program is to maximize the joint entropy of the query variables and its constraints are the Shannon information inequalities and new information inequalities involving $\ell_p$-norms of the degree sequences of the join attributes. The bounds based on arbitrary norms can be asymptotically lower than those based on the $\ell_1$ and $\ell_\infty$ norms, which capture the cardinalities and respectively the max-degrees of the input relations. They come with a matching query evaluation algorithm, are computable in exponential time in the query size, and are provably tight when each degree sequence is on one join attribute.

==> lower-bound.tex <==
\section{Computing the Bound}
\label{sec:bounds}

In this section we prove Theorem~\ref{th:main:bound:dual:informal}.
Recall that the main problem in our paper,
problem~\ref{problem:upper:bound}, asks for an upper bound to the
query's output, given a set of concrete statistics on the database.
So far we have proven Theorem~\ref{th:main:bound}, which says that,
for any valid information inequality of the form~\eqref{eq:ii:lp}, we
can infer {\em some} bound.  The best bound is their minimum, over all
valid inequalities~\eqref{eq:ii:lp}, and depends on the concrete
statistics of the database.  In this section we describe how to
compute the best bound, by using the dual of information inequalities.
%  by using formula~\eqref{eq:main-bound}.

% In this section we first introduce two flavors of our bound: the almost-entropic bound and the polymatroid bound. We then show that the almost-entropic bound is tight {\em asymptotically}, which is a somewhat weak notion of tightness, while the polymatroid is not tight even under this weaker notion.

% \subsection{The Almost-Entropic and Polymatroid Bounds}

% We restate Problem~\ref{problem:upper:bound} in terms of entropic
% and polymatroid vectors, using the correspondence mentioned at the
% end of Sec.~\ref{sec:background}.

Given a vector $\bm h \in \Rp^{2^{[n]}}$ an abstract conditional
$\sigma = (\bm V|\bm U)$, and an abstract statistics
$\tau = (\sigma, p)$, we denote by:
%
\begin{align}
  h(\sigma) \defeq & h(\bm V|\bm U) & h(\tau) \defeq \frac{1}{p}h(\bm U) + h(\bm V|\bm U)\label{eq:h:sigma:tau}
\end{align}
%
We say that a vector $\bm h$ {\em satisfies} a concrete log-statistics
$(\tau, b)$ if $h(\tau) \leq b$. Similarly, $\bm h\in \Rp^{2^{[n]}}$
{\em satisfies} a set of concrete log-statistics $(\Sigma, \bm b)$, in
notation $\bm h \models (\Sigma, \bm b)$, if $h(\tau_i)\leq b_i$ for
all $\tau_i \in \Sigma, b_i \in \bm b$.

\begin{defn} \label{def:primal:dual:bounds:k} If $\Sigma=\set{\tau_1,\ldots,\tau_s}$ is a set of
  abstract statistics, then a {\em $\Sigma$-inequality} is an
  information inequality of the form:
%
  \begin{align}
    \sum_{i \in [s]} w_i h(\tau_i) \geq & h(\bm X) \label{eq:ii:lp:revisited}
  \end{align}
%
  where $w_i \geq 0$.  Notice that~\eqref{eq:ii:lp} in
  Theorem~\ref{th:main:bound} is a $\Sigma$-inequality.
  
  For $K \subseteq \Rp^{2^{[n]}}$, the log-upper bound and log-lower
  bound of a set of log-statistics $(\Sigma,\bm b)$ are:
  %
  \begin{align}
    \text{Log-U-Bound}_K(\Sigma,\bm b) \defeq & \inf_{\bm w: K\models \text{Eq.~\eqref{eq:ii:lp:revisited}}}\sum_{i\in[s]} w_i b_i\label{eq:u:bound}\\
    \text{Log-L-Bound}_K(\Sigma,\bm b) \defeq & \sup_{\bm h \in K: \bm  h\models (\Sigma,\bm b)}h(\bm X)\label{eq:l:bound}
  \end{align}
\end{defn}
%

Fix a query $Q(\bm X) = \bigwedge_j R_j(\bm Y_j)$ that guards
$\Sigma$, and assume $K = \bar \Gamma_n^*$: by
Theorem~\ref{th:main:bound}, if a database $\bm D$ satisfies the
statistics $(\Sigma, \bm B)$, then
$\log |Q(\bm D)| \leq \text{Log-U-Bound}_K$, but it is an open problem
whether this bound is computable.  On the other hand,
$\text{Log-L-Bound}_K$ is not a bound, but it has two good properties.
First, when $K=\Gamma_n$, then $\text{Log-L-Bound}_K$ {\em is}
computable, as the optimal value of a linear program: we show this in
Example~\ref{ex:linear:optimization}.  Second, when the optimal vector
$\bm h^*$ of the maximization problem~\eqref{eq:l:bound} is the
entropy of some relation, then we can construct a ``worst-case
database instance'' $\bm D$: we use this in
Sec.~\ref{sec:simple:inequalities}.  We prove that~\eqref{eq:u:bound}
and~\eqref{eq:l:bound} are equal:

\begin{thm} \label{th:u:eq:l} If $K$ is any closed, convex cone, and
  $N_n \subseteq K \subseteq \Gamma_n$ then
  $\text{Log-U-Bound}_K=\text{Log-L-Bound}_K$.
\end{thm}

The special case of this theorem when $K=\Gamma_n$ was already
implicit in~\cite{DBLP:conf/pods/Khamis0S17}.  The proof of the
general case is more difficult, and we defer it to~\cite{arxiv-version}.  Both $\bar \Gamma_n^*$ and $\Gamma_n$
are closed, convex cones, hence the theorem applies to both.  We call
the corresponding bounds the {\em almost-entropic bound} (when
$K = \bar \Gamma_n^*$) and the {\em polymatroid bound} (when
$K = \Gamma_n$) respectively.

% The intuition behind the theorem is that it gives us an alternative,
% and more effective way to search for the best bound of a query.  The
% upper bound~\eqref{eq:u:bound} corresponds to a naive way of applying
% Theorem~\ref{th:main:bound}: try out all vectors $\bm w$ that form a
% valid inequality~\eqref{eq:ii:lp:revisited}, and return the minimum
% value of $\sum_\tau w_\tau b_\tau$, which is the logarithm of
% quantity~\eqref{eq:bound:lp}.  In particular,
% Theorem~\ref{th:main:bound} implies:
% %
% \begin{align*}
%   \text{If } \bm D \models & (\Sigma, \bm B) & \text{ then } \log |Q(\bm D)| \leq & \text{Log-U-Bound}_{\bar \Gamma_n^*}(Q,\Sigma,\bm b)
% \end{align*}
% %
% In contrast, the lower bound~\eqref{eq:l:bound}, corresponds to
% finding an entropic vector $\bm h$ that satisfies all statistics and
% maximizes $h(\bm X)$.  One should think of $\bm h$ as a proxy for a
% database instance $\bm D$, using the correspondence at the end of
% Sec.~\ref{sec:background}, s.t. $h(\bm X)=\log |Q(\bm D)|$: the lower
% bound asks us to find $\bm D$ that maximizes $|Q(\bm D)|$.  It is open
% how to find an optimal entropic vector $\bm h$, but we can compute an
% optimal polymatroid $\bm h$ using a linear program.  The theorem
% implies both the entropic and polymatroid upper and lower bounds
% coincide:
% %
% \begin{align*}
%   \text{Log-L-Bound}_{\bar \Gamma_n^*}(Q,\Sigma,\bm b)= & \text{Log-U-Bound}_{\bar \Gamma_n^*}(Q,\Sigma,\bm b)\\
%   \text{Log-L-Bound}_{\Gamma_n}(Q,\Sigma,\bm b)= & \text{Log-U-Bound}_{\Gamma_n}(Q,\Sigma,\bm b)
% \end{align*}
% %
% Also,
% $\text{Log-U-Bound}_{\bar \Gamma_n^*}(Q,\Sigma,\bm b) \leq
% \text{Log-U-Bound}_{\Gamma_n}(Q,\Sigma,\bm b)$ because
% $\bar \Gamma_n^* \subseteq \Gamma_n$.  Thus, the almost-entropic bound
% is better, but it is an open problem whether it is computable, while
% the polymatroid bound is computable.

There are two important applications of Theorem~\ref{th:u:eq:l}.
First, it gives us an effective algorithm for computing the
polymatroid bound, by computing the optimal value of a linear program:
we used this method in all experiments in
the full version~\cite{arxiv-version}.  We illustrate here with a simple
example.

\begin{ex} \label{ex:linear:optimization}
  Consider the triangle query $Q$ in~\eqref{eq:triangle:query:intro}.
  Assume that we have the following statistics for the relations
  $R, S, T$: (a) their cardinalities, denoted by $B_R, B_S, B_T$,
  whose logarithms are $b_R, b_S, b_T$, (b) the $\ell_2$-norms of all
  degree sequences: (c) the $\ell_3$ norms of all degree sequences.
  Then the polymatroid bound~\eqref{eq:l:bound} can be computed by
  optimizing the following linear program, with 8 variables
  $h(\emptyset),h(X),\ldots,h(XYZ)$:
  %
  \begin{align*}
    & \text{maximize } h(XYZ), \text{ subject to:}\\
    &\hspace*{1em} h(XY) \leq b_R,\ h(YZ) \leq b_S\ h(XZ)\leq b_T &&\text{// cardinality stats}\\
    &\hspace*{1em} \frac{1}{2}h(X)+h(Y|X)\leq b_{((Y|X),2)}\ \ \ \ \ldots  &&\text{// $\ell_2$-norm stats}\\
    &\hspace*{1em} \frac{1}{3}h(X)+h(Y|X) \leq b_{((Y|X),3)}\ \ \ \ \ldots &&\text{// $\ell_3$-norms stats}\\
    &\hspace*{1em} h(X)+h(XYZ) \leq h(XY)+h(XZ)   &&\text{// Shannon inequalities} \\
    &\hspace*{1em} h(Y)+h(XYZ) \leq h(XY)+h(YZ)\ \ \ \ &&\text{// i.e.~\eqref{eq:emptyset:zero}-\eqref{eq:submodularity}}\\
    &\hspace*{1em} \ldots
  \end{align*}
  %
\end{ex}

The second application of Theorem~\ref{th:u:eq:l} is that it allows us
to reason about the tightness of the bounds.  If we can convert the
optimal $\bm h^*$ in the lower bound~\eqref{eq:l:bound} into a
database, then we have a worst-case instance witnessing the fact that
the bound is tight.  We show in the full version~\cite{arxiv-version}
that the almost-entropic bound is {\em asymptotically} tight (a weaker
form of tightness), while the polymatroid bound is not tight.
However, we show in the next section that the polymatroid bound is
tight in the special case of simple degrees.



